Surrogate Gap Minimization Improves Sharpness-Aware Training

The recently proposed Sharpness-Aware Minimization (SAM) improves generalization by minimizing a \textit{perturbed loss} defined as the maximum loss within a neighborhood in the parameter space. However, we show that both sharp and flat minima can have a low perturbed loss, implying that SAM does not always prefer flat minima. Instead, we define a \textit{surrogate gap}, a measure equivalent to the dominant eigenvalue of Hessian at a local minimum when the radius of the neighborhood (to derive the perturbed loss) is small. The surrogate gap is easy to compute and feasible for direct minimization during training. Based on the above observations, we propose Surrogate \textbf{G}ap Guided \textbf{S}harpness-\textbf{A}ware \textbf{M}inimization (GSAM), a novel improvement over SAM with negligible computation overhead. Conceptually, GSAM consists of two steps: 1) a gradient descent like SAM to minimize the perturbed loss, and 2) an \textit{ascent} step in the \textit{orthogonal} direction (after gradient decomposition) to minimize the surrogate gap and yet not affect the perturbed loss. GSAM seeks a region with both small loss (by step 1) and low sharpness (by step 2), giving rise to a model with high generalization capabilities. Theoretically, we show the convergence of GSAM and provably better generalization than SAM. Empirically, GSAM consistently improves generalization (e.g., +3.2\% over SAM and +5.4\% over AdamW on ImageNet top-1 accuracy for ViT-B/32). Code is released at \url{ https://sites.google.com/view/gsam-iclr22/home}.

==> figure_ablation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/ablations.pdf}
    \caption{Top-1 accuracy of ViT-B/32 for the additional studies (Section~\ref{sec:ablation}). \textbf{Left}: from left to right are performances under different data augmentations (details in Appendix~\ref{sec:appendix_aug})
    %\boqing{No text explains Light, Medium, or Strong. Probably describe them here or in the main text}
    , where vanilla method is trained for $2\times$ the epochs. \textbf{Right}: performance with different base optimizers. %\textbf{Right}: comparison between GSAM and minimizing a weighted combination of the objectives in Eq.~\ref{eq:GAD_objective}%\boqing{Could we update the title of the figure to ``Improvement over weighted combination''? We have used vanilla training to refer to SGD already, so better not give it another meaning in the same paper.}
    .}
    \label{fig:ablation}
    \vspace{-4mm}
\end{figure}

==> fp_converge2.tex <==
In this section, we provide a proof for the convergence of GSAM without replying on the L-smoothness of $f_p$. 

By $L-$smoothness of $f$ and the definition of $f_p (w_t) = f(w^{adv}_t)$, and definition of $d_t = w_{t+1}-w_t$ and $w^{adv}_t = w_t + \delta_t$ we have
\begin{align}
    f_p(w_{t+1}) &= f(w^{adv}_{t+1}) \leq f(w^{adv}_t) + \langle \nabla f(w^{adv}_t), w^{adv}_{t+1} - w^{adv}_t \rangle + \frac{L}{2} \Big \vert \Big \vert w^{adv}_{t+1}-w^{adv}_t \Big \vert \Big \vert^2 \\
    &= f(w_t^{adv}) + \langle \nabla f(w_t^{adv}), w_{t+1}+\delta_{t+1}-w_t-\delta_t \rangle \nonumber \\
    &+ \frac{L}{2} \Big \vert \Big \vert w_{t+1}+\delta_{t+1}-w_t-\delta_t \Big \vert \Big \vert^2 \\
    &\leq f(w^{adv}_{t}) + \langle \nabla f(w^{adv}_t), d_t \rangle + L  \Big \vert \Big \vert  d_t  \Big \vert \Big \vert^2 \label{speq:same_part} \\
    &+ \langle  \nabla f(w_t^{adv}), \delta_{t+1}-\delta_t  \rangle + L \Big \vert \Big \vert \delta_{t+1}-\delta_t \Big \vert \Big \vert^2 \label{supeq:dif_part}
\end{align}
It's trivial to see that Eq.~\ref{speq:same_part} has the same form as Eq.~\ref{supeq:one_step_bound}, except the constant $L_p$ is replaced with a constant $2L$ which is even better bounded, so we can reuse RHS of Eq.~\ref{supeq:bound2} by replacing $L_p$ with $2L$. Now we focus on the difference caused by Eq.~\ref{supeq:dif_part}.

By definition of $\delta_t$, we have
\begin{align}
    \delta_t &= \rho_t \frac{g^{(t)}}{\vert \vert g^{(t)} \vert \vert+\epsilon} \\
    \delta_{t+1} &= \rho_{t+1} \frac{ g^{(t+1)} }{\vert \vert g^{(t+1)} \vert \vert+\epsilon}
\end{align}
where $g^{(t)}$ is the gradient of $f$ at $w_t$ evaluated with a noisy data sample. When learning rate $\eta_t$ is small, the update in weight $d_t$ is small, and expected gradient is
\begin{equation}
    \nabla f(w_{t+1}) =\nabla f(w_t + d_t) = \nabla f(w_t) + H d_t + O(\vert \vert d_t \vert \vert^2)
\end{equation}
where $H$ is the Hessian at $w_t$.
Therefore, we have
\begin{align}
    \mathbb{E} \langle \nabla f(w^{adv}_t), \delta_{t+1}-\delta_t \rangle &= \langle \nabla f(w^{adv}_t) , \rho_t \mathbb{E} \frac{g^{(t)}}{\vert \vert g^{(t)} \vert \vert+\epsilon} - \rho_{t+1} \mathbb{E} \frac{g^{(t+1)}}{\vert \vert g^{(t+1)} \vert \vert+\epsilon} \rangle \label{supeq:bound3} \\
    &\leq \vert \vert \nabla f(w_t^{adv}) \vert \vert  \rho_t \Big \vert \Big \vert \mathbb{E} \frac{g^{(t)}}{\vert \vert g^{(t)} \vert \vert+\epsilon} - \mathbb{E} \frac{g^{(t+1)}}{\vert \vert g^{(t+1)} \vert \vert+\epsilon} \Big \vert \Big \vert \\
 &\leq \vert \vert \nabla f(w_t^{adv}) \vert \vert \rho_t \phi_t \label{supeq:bound4}
\end{align}
where the first inequality is due to (1) $\rho_t$ is monotonically decreasing with $t$, and (2) triangle inequality that $ \langle a, b \rangle \leq \vert \vert a
 \vert \vert \cdot \vert \vert b \vert \vert $.
$\phi_t$ is the angle between the unit vector in the direction of $\nabla f(w_t)$ and $\nabla f(w_{t+1})$. The second inequality comes from that (1) $\Big \vert \Big \vert \frac{g}{\vert \vert g \vert \vert+\epsilon} \Big \vert \Big \vert< 1$ strictly, so we can replace $\delta_t$ in Eq.~\ref{supeq:bound3} with a unit vector in corresponding directions multiplied by $\rho_t$ and get the upper bound, (2) the norm of difference in unit vectors can be upper bounded by the arc length  on a unit circle.

When learning rate $\eta_t$ and update stepsize $d_t$ is small, $\phi_t$ is also small.
Using the limit that
\begin{equation}
    \operatorname{tan}x=x+O(x^2), \ \ \ \ \operatorname{sin}x=x+O(x^2), \ \ \ \ x \to 0 \nonumber
\end{equation}
We have:
\begin{align}
     \operatorname{tan} \phi_t &= \frac{\vert \vert \nabla f(w_{t+1}) - \nabla f(w_t) \vert \vert}{\vert \vert \nabla f(w_{t}) \vert \vert} + O(\phi_t^2) \\
    &= \frac{\vert \vert H d_t + O(\vert \vert d_t \vert \vert^2) \vert \vert}{\vert \vert \nabla f(w_{t}) \vert \vert} + O(\phi_t^2) \\
    &\leq \eta_t L (1+\alpha)
\end{align}
where the last inequality is due to (1) max eigenvalue of $H$ is upper bounded by $L$ because $f$ is $L-$smooth, (2) $\vert \vert d_t \vert \vert = \vert \vert \eta_t (g_\parallel + \alpha g_\perp) \vert \vert$ and $\mathbb{E} g_t = \nabla f(w_t)$.

Plug into Eq.~\ref{supeq:bound4}, also note that the perturbation amplitude $\rho_t$ is small so $w_t$ is close to $w^{adv}_t$, then we have
\begin{equation}
    \mathbb{E} \langle \nabla f(w^{adv}_t), \delta_{t+1}-\delta_t \rangle \leq L (1+\alpha) G \rho_t \eta_t \label{supeq:bound6}
\end{equation}
Similarly, we have
\begin{align}
    \mathbb{E} \Big \vert \Big \vert \delta_{t+1}-\delta_t \Big \vert \Big \vert^2 &\leq \rho_t^2 \mathbb{E} \Big \vert \Big \vert \frac{g^{(t)}}{\vert \vert g^{(t)} \vert \vert+\epsilon} - \frac{g^{(t+1)}}{\vert \vert g^{(t+1)} \vert \vert+\epsilon}   \Big \vert \Big \vert^2 \\
    &\leq \rho_t^2 \phi_t^2 \\
    &\leq \rho_t^2 \eta_t^2 L^2 (1+\alpha)^2 \label{supeq:bound7}
\end{align}
Reuse results from Eq.~\ref{supeq:bound2} (replace $L_p$ with $2L$) and plug into Eq.~\ref{speq:same_part}, and plug Eq.~\ref{supeq:bound6} and Eq.~\ref{supeq:bound7} into Eq.~\ref{supeq:dif_part}, we have
\begin{align}
\mathbb{E} f_p(w_{t+1}) - f_p(w_t)
    &\leq -\eta_t \mathbb{E} \Big \vert \Big \vert \nabla f_p(w_t) \Big \vert \Big \vert_2^2 + \frac{2L (\alpha+1)^2}{2}G^2 \eta_t^2 \nonumber \\
    &+ L(1+\alpha)G\rho_t \eta_t + \frac{2L^3 (1+\alpha)^2}{2} \eta_t^2 \rho_t^2
\end{align}
Perform telescope sum, we have
\begin{align}
    \mathbb{E} f_p(w_T) - f_p(w_0) &\leq -\sum_{t=1}^T \eta_t \mathbb{E} \vert \vert \nabla f_p(w_t) \vert \vert^2 + \Big[ L(1+\alpha)^2 G^2 \eta_0^2 + L(1+\alpha)G \rho_0 \eta_0 \Big] \sum_{t=1}^T \frac{1}{t} \nonumber \\
    &+ L^3(1+\alpha)^2 \eta_0^2 \rho_0^2 \sum_{t=1}^T \frac{1}{t^2}
\end{align}
Hence
\begin{align}
    \eta_T \sum_{t=1}^T \mathbb{E} \vert \vert \nabla f_p(w_t) \vert \vert^2 \leq  \sum_{t=1}^T \eta_t \mathbb{E} \vert \vert \nabla f_p(w_t) \vert \vert^2 \leq f_p(w_0) - \mathbb{E}f_p(w_T)  + D \log T +  \frac{\pi^2 E}{6}
\end{align}
where
\begin{equation}
    D = L(1+\alpha)^2 G^2  \eta_0^2 + L(1+\alpha) G \rho_0 \eta_0,\ \ \ \  E = L^3(1+\alpha)^2 \eta_0^2 \rho_0^2
\end{equation}
Note that $\eta_T = \frac{\eta_0}{\sqrt{T}}$, we have
\begin{equation}
    \frac{1}{T}\sum_{t=1}^T \mathbb{E} \vert \vert \nabla f_p(w_t) \vert \vert^2 \leq \frac{f_p(w_0)-f_{min}+\pi^2 E /6}{\eta_0} \frac{1}{\sqrt{T}} + \frac{D}{\eta_0} \frac{\log T}{\sqrt{T}}
\end{equation}
which implies that GSAM converges at a rate of $O(\log T /\sqrt{T})$, and all the constants here are well-bounded.

==> fp_converge_0.tex <==
By $L-$smoothness of $f(w)$, we have
\begin{equation}
    \vert \vert \nabla f(w_1) - \nabla f(w_2) \vert \vert \leq L \vert \vert w_1 - w_2 \vert \vert
\end{equation}
Hence we can derive the smoothness of $f_p(w)$
\begin{align}
   \Big \vert \Big \vert \nabla f_p(w_1) - \nabla f_p(w_2) \Big \vert \Big \vert &= \Big \vert \Big \vert \nabla f \Big(w_1 + \rho \frac{\nabla f(w_1)}{\vert \vert \nabla f(w_1) \vert \vert+\epsilon} \Big ) - \nabla f \Big(w_2 + \rho \frac{\nabla f(w_2)}{\vert \vert \nabla f(w_2) \vert \vert+\epsilon} \Big ) \Big \vert \Big \vert \\
   &\leq L \Big \vert \Big \vert \Big(w_1 + \rho \frac{\nabla f(w_1)}{\vert \vert \nabla f(w_1) \vert \vert+\epsilon} \Big ) - \Big(w_2 + \rho \frac{\nabla f(w_2)}{\vert \vert \nabla f(w_2) \vert \vert+\epsilon} \Big ) \Big \vert \Big \vert \\
   &\Big( f \text{ is Lipschitz} \Big) \nonumber \\
   &\leq L \Big \vert \Big \vert w_1 - w_2 \Big \vert \Big \vert + L \rho \Big \vert \Big \vert \frac{\nabla f(w_1)}{\vert \vert \nabla f(w_1) \vert \vert + \epsilon} -  \frac{\nabla f(w_2)}{\vert \vert \nabla f(w_2) \vert \vert + \epsilon} \Big \vert \Big \vert \\
   &\leq L \Big \vert \Big \vert w_1 - w_2 \Big \vert \Big \vert + \frac{L\rho}{\epsilon} \Big \vert \Big \vert \nabla f(w_1) - \nabla f(w_2) \Big \vert \Big \vert \\
   &\Big ( \frac{x}{\vert \vert x \vert \vert + \epsilon} \text{ is Lipschitz-continuous with constant $\frac{1}{\epsilon}$} \Big) \nonumber \\
   &\leq \Big( L + \frac{L^2 \rho}{\epsilon} \Big) \Big \vert \Big \vert w_1 - w_2 \Big \vert \Big \vert \\
   &\Big( f \text{ is Lipschitz} \Big) \nonumber
\end{align}
Hence we prove the smoothness of $f_p$. %(except on the set of isolated local minimum whose measure is 0).
For simplicity, we denote $L_p = L + \frac{L^2 \rho}{\epsilon}$ as the Lipschitz constant of $f_p(w)$.

For simplicity of notation, we denote the update at step $t$ as
\begin{equation}
    d_t = -\eta_t g_p^{(t)} + \eta_t \alpha g^{(t)}_\perp
\end{equation}
By smoothness of $f_p(w)$, we have
\begin{align}
    f_p(w_{t+1}) &\leq f_p(w_t) + \langle \nabla f_p(w_t), d_t \rangle + \frac{L_p}{2} \Big \vert \Big \vert d_t \Big \vert \Big \vert^2_2 \label{supeq:one_step_bound} \\
    &= f_p(w_t) + \langle \nabla f_p(w_t), -\eta_t g_p^{(t)} + \alpha \eta_t g^{(t)}_\perp \rangle + \frac{L_p}{2} \Big \vert \Big \vert d_t \Big \vert \Big \vert^2_2
\end{align}
Take expectation conditioned on observation up to step $t$ (for simplicity of notation, we use $\mathbb{E}$ short for $\mathbb{E}_x$ to denote expectation over all possible data points) conditioned on observations up to step $t$, we have 
\begin{align}
    \mathbb{E} f_p(w_{t+1}) - f_p(w_t) &\leq -\eta_t \langle \nabla f_p(w_t), \mathbb{E} g_p^{(t)} \rangle + \alpha \eta_t \langle \nabla f_p(w_t), \mathbb{E} g^{(t)}_\perp \rangle \nonumber \\
    & + \frac{L_p}{2} \eta_t^2 \mathbb{E} \Big \vert \Big \vert -g_p^{(t)} + \alpha g_\perp^{(t)} \Big \vert \Big \vert_2^2 \\
    &\leq -\eta_t \mathbb{E} \Big \vert \Big \vert \nabla f_p(w_t) \Big \vert \Big \vert_2^2 + 0 + \frac{L_p (\alpha+1)^2}{2}G^2 \eta_t^2 \label{supeq:bound2} \\
    &\Big( \text{Since } \mathbb{E}g^{(t)}_\perp \text{ is orthogonal to } \nabla f_p(w_t) \text{ by construction}, \nonumber \\
    &\vert \vert g^{(t)} \vert \vert \leq G \text{ by assumption} \Big) \nonumber 
\end{align}
Hence we have
\begin{equation}
    \eta_t \mathbb{E} \Big \vert \Big \vert \nabla f_p(w_t) \Big \vert \Big \vert_2^2 \leq f_p(w_t) - \mathbb{E} f_p(w_{t+1}) + \frac{L_p (\alpha+1)^2G^2}{2} \eta_t^2
\end{equation}
By telescope sum, we have:
\begin{equation}
    \sum_{t=1}^T \eta_t \mathbb{E} \Big \vert \Big \vert \nabla f_p(w_t) \Big \vert \Big \vert_2^2 \leq f_p(w_0)-\mathbb{E} f_p(w_T) + \frac{L_p (\alpha+1)^2G^2}{2} \sum_{t=1}^T \eta_t^2
\end{equation}
Since $\eta_t = \eta_0 / \sqrt{t}$, we have
\begin{align}
    \frac{\eta_0}{\sqrt{T}} \sum_{t=1}^T \mathbb{E} \Big \vert \Big \vert \nabla f_p(w_t) \Big \vert \Big \vert_2^2 &\leq LHS \leq RHS \\
    &\leq f_p(w_0) - f_{min} + \frac{L_p(1+\alpha)^2G^2 \eta_0^2}{2}\Big( 1+\log T \Big) \\
\end{align}
Hence 
\begin{align}
    \frac{1}{T} \sum_{t=1}^T \mathbb{E} \Big \vert \Big \vert \nabla f_p(w_t) \Big \vert \Big \vert_2^2 &\leq \Big [ \frac{f_p(w_0)-f_{min}}{\eta_0} + \frac{L_p(1+\alpha)^2G^2 \eta_0^2}{2}\Big( 1+\log T \Big ) \Big] / \sqrt{T} \\
    &= \frac{C_1 + C_2 \log T}{\sqrt{T}}
\end{align}
where $C_1, C_2$ are some constants.
This implies that the regret w.r.t $f_p(w)$ converges at rate $O(\log T / \sqrt{T})$.

==> intro_1.tex <==
Modern neural networks are typically highly over-parameterized hence easy to overfit to training data, yet the generalization performances on unseen data (test set) typically suffer from a gap from the training performance \citep{zhang2017understanding}. Many studies try to understand the generalization of machine learning models, including the Bayesian perspective \citep{mcallester1999pac, neyshabur2017pac}, the information perspective \citep{liang2019fisher}, the geometry of loss surface \citep{hochreiter1995simplifying, jiang2019fantastic} and the kernel perspective \citep{jacot2018neural, wei2019regularization}. Besides analyzing the properties of a model after training, other works studies the influence of training and optimization process, such as the implicit regularization of stochastic gradient descent (SGD) \citep{bottou2010large, zhou2020towards}, the regularization effect of learning rate \citep{li2019towards} and the influence of batch size \citep{keskar2016large}.

Besides aforementioned works on theoretical analysis of generalization behavior, many techniques have been proposed to improve the generalization, and be broadly categorized into three types: data augmentation, model regularization and modified training schemes. Data augmentation typically generates new data from training samples; besides standard data augmentation such as flipping or rotation of images, recent data augmentations include label smoothing \citep{muller2019does} and mixup \citep{muller2019does} which trains on convex combination of both inputs and labels, automatically learned augmentation \citep{cubuk2018autoaugment}, and cutout \citep{devries2017improved} which randomly masks out part of an image. Model regularization typically applies auxiliary losses besides the training loss or randomly modifies the model architecture during training, such as decoupled weight decay \citep{loshchilov2017decoupled}, dropout \citep{srivastava2014dropout} and shake-shake regularization \citep{gastaldi2017shake}. Note that data augmentation and model regularization literatures mentioned here typically train with the standard back-propagation \citep{rumelhart1985learning} and first-order gradient optimizers such as SGD \citep{bottou2010large} and Adam \citep{kingma2014adam}.

Different from data augmentation and model regularization, another research direction is to modify the training scheme to improve generalization. \cite{keskar2017improving} proposed to use Adam in the early phases for fast convergence, then switch to SGD for better generalization. \cite{izmailov2018averaging} proposed to average weights to achieve a wider local minima, and similar idea is later used in Lookahead \citep{zhang2019lookahead}. Entropy-SGD \citep{chaudhari2019entropy} derives the gradient of local entropy (rather than gradient on a single point of parameter weights), and seeks a wider valley which is expected to have better generalization. However, Entropy-SGD has a nested loop within the training process to approximate the entropy within a neighborhood, hence has a much larger computation cost than vanilla training. 

The recently proposed Sharpness Aware Minimization (SAM) \citep{foret2020sharpness} is a generic training scheme that improves generalization, and has been validated when pre-training is unavailable \citep{chen2021vision}. 
%Its variant Adaptive-SAM \citep{kwon2021asam} tackles the sensitivity of SAM to re-scaling of neural networks.
Vanilla training minimizes the loss $f(w)$ where $w$ is the weight of parameters, while SAM minimizes the \textit{perturbed loss} defined as $f_r(w) \triangleq \operatorname{max}_{\vert \vert \delta \vert \vert \leq \rho} f(w+\delta)$, which is the \textit{maximum} loss within radius $\rho$ centered at $w$. Intuitively, vanilla training seeks a single point with a low loss, while SAM seeks for a neighborhood within which the maximum loss is low (hence the average loss is low). However, when $\rho$ is not properly chosen SAM might prefer a sharp local minima: for the toy example in Fig.~\ref{fig: gap_toy} (a), $w_1$ is sharper than $w_2$, but SAM would prefer $w_1$ because it has a lower perturbed loss $f_r(w_1) < f_r(w_2)$. Therefore, a low $f_r$ could appear in both flat and sharp minima, and minimizing $f_r$ not always ends up in a wide valley.

Although $f_r(w)$ might disagree with sharpness, we found the \textit{surrogate gap} defined as $h(w) \triangleq f_r(w)-f(w)$ agrees with flatness (e.g. for any fixed $\rho$ that does not exceed the width of valley, a low $h$ always represent a flat minima, as shown in Fig.~\ref{fig: gap_toy}). Inspired by this observation, we propose Gradient Decomposition Descent Ascent (GDDA), which seeks a neighborhood with both a low loss value (by minimizing $f_r$) and a low sharpness (by minimizing $h$). A low $f_r$ indicates a low training loss within the neighborhood, and a low $h$ indicates a smaller generalization gap between training performance and test performance.

\begin{figure}
\begin{subfigure}{0.47\textwidth}
\includesvg[width=\linewidth]{figures/gap_toy3.svg}
\caption{Case 1, perturbation amplitude $\rho$ is small.}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\textwidth}
\includesvg[width=\linewidth]{figures/gap_toy2.svg}
\caption{Case 2, perturbation amplitude $\rho$ is large.}
\end{subfigure}

%\caption{Consider two local minima $w_1$ and $w_2$, where loss surface around $w_1$ is sharper than $w_2$. Consider training loss $f$ (solid line), perturbed loss $f_r \triangleq \operatorname{max}_{\vert \vert \delta \vert \vert \leq \rho} f(w+\delta)$ (dash line), and surrogate gap $h(w) \triangleq f_r(w)-f(w)$. Intuitively, $f_r$ is a smoothed version of $f$ convolved with a kernel of width $2\rho$. Note that (a) and (b) have the same $f$ (solid lines) but different $\rho$ hence different $f_r$ (dash lines). (a) When perturbation amplitude $\rho$ is small, $f$ is close to $f_r$, and $f_r(w_1) < f_r(w_2)$, SAM will prefer $w_1$ since it's minimizing $f_r$. (b) When perturbation amplitude $\rho$ is large, $f$ is distant from $f_r$, and $f_r(w_1) > f_r(w_2)$, SAM will prefer $w_2$. Comparing (a) and (b), perturbed loss $f_r$ is sensitive to $\rho$, and a lower $f_r$ does not imply a flatter surface (e.g. the relative magnitude between $f_r(w_1)$ and $f_r(w_2)$ is flipped in (a) and (b), even though $f$ is the same), hence SAM not always choose a wide valley. However, for any fixed $\rho$ that is smaller than width of the valley, a smaller $h$ always represent a flatter minima, e.g. $h(w_1)>h(w_2)$ for both (a) and (b). Note: in Sec. we show that with a carefully chosen larger $\rho$, SAM is still inferior to the proposed method, because SAM only minimizes $f_r$ hence seeks for neighborhood with a low loss, while the proposed method proactively minimizes both $f_r$ and $h$ hence seeks for neighborhood with both low loss and small sharpness.}

\caption{Consider two local minima $w_1$ and $w_2$, where loss surface around $w_1$ is sharper than $w_2$. Consider training loss $f$ (solid line), perturbed loss $f_r \triangleq \operatorname{max}_{\vert \vert \delta \vert \vert \leq \rho} f(w+\delta)$ (dash line), and surrogate gap $h(w) \triangleq f_r(w)-f(w)$. Intuitively, $f_r$ is a smoothed version of $f$ convolved with a kernel of width $2\rho$. Note that (a) and (b) have the same $f$ (solid lines) but different $\rho$ hence different $f_r$ (dash lines). As summarized in Table.~\ref{table: toy}, a lower $f_r$ does not imply a flatter minima, e.g. $f_r(w_1)<f_r(w_2)$ in (a) but $f_r(w_1)>f_r(w_2)$ in (b), even though the loss surface for $f$ is the same for (a) and (b). Different from $f_r$, the surrogate gap $h$ is a consistent measure for flatness, and $h(w_1)>h(w_2)$ for both cases.}
\label{fig: gap_toy}
\end{figure}

\begin{table}[]
\caption{Comparison on the toy example in Fig.~\ref{fig: gap_toy}.} \label{table: toy}
\begin{tabular}{c|cccc}
\hline
                      & relative relation of $f_r$ & relative relation of $h$ & relative relation of flatness  &  SAM solution\\ \hline
Fig 1. (a) &   $f_r(w_1)<f_r(w_2)$   & $h(w_1)>h(w_2)$   &   $w_2$ flatter than $w_1$   &  $w_1$        \\
Fig 1. (b) &    $f_r(w_1)>f_r(w_2)$  &  $h(w_1) > h(w_2)$  &    $w_2$ flatter than $w_1$    & $w_2$        \\ \hline
\end{tabular}
\end{table}


==> table_imagenet_all_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Top-1 Accuracy (\%) on ImageNet datasets for ResNets, ViTs and MLP-Mixers trained with Vanilla SGD or AdamW, SAM, and GSAM optimizers.
}\label{table:imagenet_all}
\centering
\scalebox{0.82}{
\begin{tabular}{ccccccc}
\shline
\multicolumn{1}{c|}{Model}                       & \multicolumn{1}{c|}{Training}    & ImageNet-v1    & ImageNet-Real & \multicolumn{1}{c|}{ImageNet-V2}   & ImageNet-R    & ImageNet-C    \\ 
\shline
\multicolumn{7}{c}{ResNet}                                                                                                                                                                \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{ResNet50}}   & \multicolumn{1}{c|}{Vanilla (SGD)}         & 76.0             & 82.4          & \multicolumn{1}{c|}{63.6}          & 22.2          & 44.6          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 76.9           & 83.3          & \multicolumn{1}{c|}{64.4}          & 23.8          & 46.5          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{77.2} & \textbf{83.9} & \multicolumn{1}{c|}{\textbf{65.2}} & \textbf{24.4} & \textbf{47.9} \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{ResNet101}}  & \multicolumn{1}{c|}{Vanilla (SGD)}         & 77.8           & 83.9          & \multicolumn{1}{c|}{65.3}          & 24.4          & 48.5          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 78.6           & 84.8          & \multicolumn{1}{c|}{66.7}          & 25.9          & 51.3          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{78.9}  & \textbf{85.2} & \multicolumn{1}{c|}{\textbf{67.1}} & \textbf{26.3} & \textbf{52.1} \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{ResNet152}}  & \multicolumn{1}{c|}{Vanilla (SGD)}         & 78.5           & 84.2          & \multicolumn{1}{c|}{66.3}          & 25.3          & 50.0            \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 79.3           & 84.9          & \multicolumn{1}{c|}{67.3}          & 25.7          & 52.2          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{79.8}  & \textbf{85.8} & \multicolumn{1}{c|}{\textbf{68.1}} & \textbf{26.8} & \textbf{53.5} \\ 
\shline

\multicolumn{7}{c}{Vision Transformer}                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{ViT-S/32}}   & \multicolumn{1}{c|}{Vanilla (AdamW)}        & 68.4           & 75.2          & \multicolumn{1}{c|}{54.3}          & 19.0         & 43.3          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 70.5           & 77.5          & \multicolumn{1}{c|}{56.9}          & 21.4          & 46.2          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{73.1}  & \textbf{80.5} & \multicolumn{1}{c|}{\textbf{59.7}} & \textbf{23.1} & \textbf{47.2} \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{ViT-S/16}}   & \multicolumn{1}{c|}{Vanilla (AdamW)}        & 74.4           & 80.4          & \multicolumn{1}{c|}{61.7}          & 20.0            & 46.5          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 78.1           & 84.1          & \multicolumn{1}{c|}{65.6}          & \textbf{24.7}          & 53.0            \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{79.5}  & \textbf{85.1} & \multicolumn{1}{c|}{\textbf{67.0}}   & 24.6 & \textbf{53.1} \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{ViT-B/32}}   & \multicolumn{1}{c|}{Vanilla (AdamW)} & 71.4           & 77.5          & \multicolumn{1}{c|}{57.5}          & 23.4          & 44.0            \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 73.6           & 80.3          & \multicolumn{1}{c|}{60.0}            & 24.0            & 50.7          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{76.8}  & \textbf{82.8} & \multicolumn{1}{c|}{\textbf{62.8}} & \textbf{25.3} & \textbf{52.0}   \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{ViT-B/16}}   & \multicolumn{1}{c|}{Vanilla (AdamW)}        & 74.6           & 79.8          & \multicolumn{1}{c|}{61.3}          & 20.1          & 46.6          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 79.9           & 85.2          & \multicolumn{1}{c|}{67.5}          & 26.4          & \textbf{56.5}          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{81.2}  & \textbf{86.6} & \multicolumn{1}{c|}{\textbf{69.3}} & \textbf{27.2} & 55.6          \\ 
\shline

\multicolumn{7}{c}{MLP-Mixer}                                                                                                                                                             \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{Mixer-S/32}} & \multicolumn{1}{c|}{Vanilla (AdamW)}        & 63.9           & 70.3          & \multicolumn{1}{c|}{49.5}          & 16.9          & 35.2          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 66.7           & 73.8          & \multicolumn{1}{c|}{52.4}          & 18.6          & 39.3          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{68.6}  & \textbf{75.8} & \multicolumn{1}{c|}{\textbf{55.4}} & \textbf{23.3} & \textbf{45.3} \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{Mixer-S/16}} & \multicolumn{1}{c|}{Vanilla (AdamW)}        & 68.8           & 75.1          & \multicolumn{1}{c|}{54.8}          & 15.9          & 35.6          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 72.9           & 79.8          & \multicolumn{1}{c|}{58.9}          & 20.1          & 42.0            \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{75.1}  & \textbf{81.9} & \multicolumn{1}{c|}{\textbf{61.8}} & \textbf{23.9} & \textbf{48.9} \\ \hline

\multicolumn{1}{l|}{\multirow{3}{*}{Mixer-S/8}}  & \multicolumn{1}{c|}{Vanilla (AdamW)}        & 70.2           & 76.2          & \multicolumn{1}{c|}{56.1}          & 15.4          & 34.6          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 75.9           & 82.5          & \multicolumn{1}{c|}{62.3}          & 20.5          & 42.4          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{76.8}  & \textbf{83.3} & \multicolumn{1}{c|}{\textbf{63.7}} & \textbf{23.6} & \textbf{48.2} \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{Mixer-B/32}} & \multicolumn{1}{c|}{Vanilla (AdamW)}        & 62.5           & 68.1          & \multicolumn{1}{c|}{47.6}          & 14.6          & 33.8          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 72.4           & 79.0            & \multicolumn{1}{c|}{58.0}            & 22.8          & 46.2          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{73.8}  & \textbf{80.0}   & \multicolumn{1}{c|}{\textbf{60.0}}   & \textbf{27.8} & \textbf{52.4} \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{Mixer-B/16}} & \multicolumn{1}{c|}{Vanilla (AdamW)}        & 66.4           & 72.1          & \multicolumn{1}{c|}{50.8}          & 14.5          & 33.8          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 77.4           & 83.5          & \multicolumn{1}{c|}{63.9}          & 24.7          & 48.8          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textbf{GSAM}}        & \textbf{78.3}  & \textbf{84.5} & \multicolumn{1}{c|}{\textbf{65.7}} & \textbf{28.7} & \textbf{55.0}   \\
\shline
\end{tabular}
}
\end{table}

==> table_imagenet_plus.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Top-1 Accuracy (\%) on ImageNet datasets for ResNet, ViT and MLP-Mixers trained with SGD/Adam, SAM and GSAM.
}\label{table:imagenet_all}
\centering
\scalebox{0.9}{
\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{Model}                       & \multicolumn{1}{c|}{Training}    & ImageNet-v1    & ImageNet-Real & \multicolumn{1}{c|}{ImageNet-V2}   & ImageNet-R    & ImageNet-C    \\ \hline
\multicolumn{7}{c}{ResNet}                                                                                                                                                                \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ResNet50}}   & \multicolumn{1}{c|}{SGD}         & 76.0             & 82.4          & \multicolumn{1}{c|}{63.6}          & 22.2          & 44.6          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 76.9           & 83.3          & \multicolumn{1}{c|}{64.4}          & 23.8          & 46.5          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{77.2(+1.2/0.3)} & \textbf{83.9(+1.5/0.6)} & \multicolumn{1}{c|}{\textbf{65.2(+1.6/0.8)}} & \textbf{24.4(+2.2/0.6)} & \textbf{47.9(+3.3/1.4)} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ResNet101}}  & \multicolumn{1}{c|}{SGD}         & 77.8           & 83.9          & \multicolumn{1}{c|}{65.3}          & 24.4          & 48.5          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 78.6           & 84.8          & \multicolumn{1}{c|}{66.7}          & 25.9          & 51.3          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{78.9(+1.1/0.3)}  & \textbf{85.2(+1.3/0.4)} & \multicolumn{1}{c|}{\textbf{67.1(+1.8/0.4)}} & \textbf{26.3(+1.9/0.4)} & \textbf{52.1(+3.6/0.8)} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ResNet152}}  & \multicolumn{1}{c|}{SGD}         & 78.5           & 84.2          & \multicolumn{1}{c|}{66.3}          & 25.3          & 50.0            \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 79.3           & 84.9          & \multicolumn{1}{c|}{67.3}          & 25.7          & 52.2          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{79.8(+1.3/0.5)}  & \textbf{85.8(+1.6/0.9)} & \multicolumn{1}{c|}{\textbf{78.1(+11.8/10.8)}} & \textbf{26.8(+1.5/1.1)} & \textbf{53.5(+3.5/1.3)} \\ \hline

\multicolumn{7}{c}{Vision-Transformer}                                                                                                                                                    \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ViT-S/16}}   & \multicolumn{1}{c|}{Adam}        & 74.4           & 80.4          & \multicolumn{1}{c|}{61.7}          & 20            & 46.5          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 78.1           & 84.1          & \multicolumn{1}{c|}{65.6}          & 24.7          & 53            \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{79.5(+5.1/0.6)}  & \textbf{85.1(+4.7/1.0)} & \multicolumn{1}{c|}{\textbf{67.0(+5.3/1.4)}}   & \textbf{24.6} & \textbf{53.1} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ViT-S/32}}   & \multicolumn{1}{c|}{Adam}        & 68.4           & 75.2          & \multicolumn{1}{c|}{54.3}          & 19            & 43.3          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 70.5           & 77.5          & \multicolumn{1}{c|}{56.9}          & 21.4          & 46.2          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{73.1}  & \textbf{80.5} & \multicolumn{1}{c|}{\textbf{59.7}} & \textbf{23.1} & \textbf{47.2} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ViT-B/16}}   & \multicolumn{1}{c|}{Adam}        & 74.6           & 79.8          & \multicolumn{1}{c|}{61.3}          & 20.1          & 46.6          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 79.9           & 85.2          & \multicolumn{1}{c|}{67.5}          & 26.4          & 56.5          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{81.2}  & \textbf{86.6} & \multicolumn{1}{c|}{\textbf{69.3}} & \textbf{27.2} & 55.6          \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ViT-B/32}}   & \multicolumn{1}{c|}{Adam} & 69.5           & 75.2          & \multicolumn{1}{c|}{55.3}          & 19.9          & 44.0            \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 73.6           & 80.3          & \multicolumn{1}{c|}{60.0}            & 24.0            & 50.7          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{76.8}  & \textbf{82.8} & \multicolumn{1}{c|}{\textbf{62.8}} & \textbf{25.3} & \textbf{52.0}   \\ \hline
\multicolumn{7}{c}{MLP-Mixer}                                                                                                                                                             \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Mixer-S/8}}  & \multicolumn{1}{c|}{Adam}        & 70.2           & 76.2          & \multicolumn{1}{c|}{56.1}          & 15.4          & 34.6          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 75.9           & 82.5          & \multicolumn{1}{c|}{62.3}          & 20.5          & 42.4          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{76.8}  & \textbf{83.3} & \multicolumn{1}{c|}{\textbf{63.7}} & \textbf{23.6} & \textbf{48.2} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Mixer-S/16}} & \multicolumn{1}{c|}{Adam}        & 68.8           & 75.1          & \multicolumn{1}{c|}{54.8}          & 15.9          & 35.6          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 72.9           & 79.8          & \multicolumn{1}{c|}{58.9}          & 20.1          & 42.0            \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{75.1}  & \textbf{81.9} & \multicolumn{1}{c|}{\textbf{61.8}} & \textbf{23.9} & \textbf{48.9} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Mixer-S/32}} & \multicolumn{1}{c|}{Adam}        & 63.9           & 70.3          & \multicolumn{1}{c|}{49.5}          & 16.9          & 35.2          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 66.7           & 73.8          & \multicolumn{1}{c|}{52.4}          & 18.6          & 39.3          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{68.6}  & \textbf{75.8} & \multicolumn{1}{c|}{\textbf{55.4}} & \textbf{23.3} & \textbf{45.3} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Mixer-B/16}} & \multicolumn{1}{c|}{Adam}        & 66.4           & 72.1          & \multicolumn{1}{c|}{50.8}          & 14.5          & 33.8          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 77.4           & 83.5          & \multicolumn{1}{c|}{63.9}          & 24.7          & 48.8          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{78.3}  & \textbf{84.5} & \multicolumn{1}{c|}{\textbf{65.7}} & \textbf{28.7} & \textbf{55.0}   \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Mixer-B/32}} & \multicolumn{1}{c|}{Adam}        & 62.5           & 68.1          & \multicolumn{1}{c|}{47.6}          & 14.6          & 33.8          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SAM}         & 72.4           & 79.0            & \multicolumn{1}{c|}{58.0}            & 22.8          & 46.2          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{GSAM}        & \textbf{73.8}  & \textbf{80.0}   & \multicolumn{1}{c|}{\textbf{60.0}}   & \textbf{27.8} & \textbf{52.4} \\ \hline
\end{tabular}
}
\end{table}
